EnclaveTree: Privacy-preserving Data Stream Training and Inference Using TEE

The classification service over a stream of data is becoming an important offering for cloud providers, but users may encounter obstacles in providing sensitive data due to privacy concerns. While Trusted Execution Environments (TEEs) are promising solutions for protecting private data, they remain vulnerable to side-channel attacks induced by data-dependent access patterns. We propose a Privacy-preserving Data Stream Training and Inference scheme, called EnclaveTree, that provides confidentiality for user's data and the target models against a compromised cloud service provider. We design a matrix-based training and inference procedure to train the Hoeffding Tree (HT) model and perform inference with the trained model inside the trusted area of TEEs, which provably prevent the exploitation of access-pattern-based attacks. The performance evaluation shows that EnclaveTree is practical for processing the data streams with small or medium number of features. When there are less than 63 binary features, EnclaveTree is up to ${\thicksim}10{\times}$ and ${\thicksim}9{\times}$ faster than na\"ive oblivious solution on training and inference, respectively.

==> sections/RF_HE.tex <==
\section{Oblivious RF Training and Inference}
\label{sub:RF_training}
\begin{table*}[htb]
\centering
\footnotesize
 \caption{Parameters setting and setup time}
 \label{table:S2}
 \begin{ThreePartTable}
    \begin{tabular}{cccccccccc}
        \toprule
        \textbf{Dimension} & \textbf{m} & \textbf{p} & \textbf{r} & \textbf{bits} & \textbf{c} & \textbf{slots} & \textbf{Security Level} & \textbf{DO (s)} & \textbf{Enclave (s)} \\
        \midrule
        16 & 9472 & 127 & 1 & 119 &  2  & 256 &  86.49 & 7.29 & 21.75 \\
        \hline
        32  & 16384 & 6143  & 1 & 180 & 2 & 1024 & 83.13 &  12.68  & 40.50 \\
        \hline
        64  & 16384  & 8191  & 1  & 120 &  2 & 4096  & 105.58 & 22.43 & 79.21 \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \centering
        \footnotesize
        \item \textbf{r}: Hensel lifting; \textbf{c}: Number of columns of Key-Switching matrix \cite{brakerski2011fully}; 
        \item \textbf{DO/Enclave}: Setup time of creating \textit{Context}, \textit{Secret Key} and \textit{Public Key} at DO and Enclave side respectively.
    \end{tablenotes}
 \end{ThreePartTable}
\end{table*}

In this section, we introduce how to extend \sys to RF training and inference in details. 
% \subsubsection{Oblivious RF Training}
% Not sure if is this paragraph necessary
% In data stream classification, the target model is supposed to be replaced with the new one when the concept drift is detected. 
% We observe that prior approaches \cite{lindell2000privacy,du2002building,vaidya2005privacy,wang2006classification,xiao2005privacy,emekcci2007privacy,samet2008privacy} raise new privacy concerns in this setting, especially when the tree is replaced with a new one. 
% Specifically, since the trees' structures or even the nodes in each path are exposed to CSP, she could compare the existing trees with a set of background trees. 
% Consequently, CSP can infer why or when the concept drift occurs and the patterns of data distribution changes. 
% Therefore, we would extend our constructions to the RF to solve this problem. 
%More details are shown on Algorithm~\ref{alg4}.

%\notegio{I thought that RF training was more than that. You ahve multiple trees, more memory required etc.}
\subsection{Oblivious RF Training}
The main difference between oblivious HT and RF training is to select a subset of features for each HT in RF. 

Specifically, enclave samples the features with replacement and randomly selects a subset of features from the feature set $S$ for each HT. 
To make the selection process oblivious, enclave access the features using $\mathtt{oaccess}$. 
The following matrix operations are similar to that in Section~\ref{sub:HT_train}.



% \textbf{m}: Cyclotomic polynomial, defines $\phi(m)$; \textbf{p}: Plaintext prime modulus; \textbf{r}: Hensel lifting; \textbf{bits}: Number of bits of the modulus chain, indicates the ability of processing noise; \textbf{c}: Number of columns of Key-Switching matrix; 

% \subsection{Oblivious RF Inference}
\subsection{SHE-based RF Inference}
\label{subsub:RF_inf}
% My logic:
% 1. inference inside the enclave (with oblivious primitives)
% 2. why do we use HE-based inference in RF
% 3. give a general look at the main operations in HE-based inference
% 4. Detail the key points in HE-based inference. 
%    First is naive solution using HE-based inner products and the shortcomings 
%    Second is our HE-based Matrix multiplications.
% 5. Parameter setting (it was in the experimental section before)
RF consists of a set of trees. 
Predicating a data instance with RF inference means classifying the instance with each tree and get a set of labels. The final predication result is the label output by the majority of trees. 
Due to the limited EPC size, the RF is encrypted and stored outside enclave. 
A straightforward method for performing RF inference is to load the trees into the enclave one by one and perform the above HT inference in plaintext within the enclave. 

However, this approach raises performance issues.

% Such an approach: 
% i) significantly increases the attack surface when using multi-threads inside the enclave \cite{khandaker2020coin,weichbrodt2016asyncshock}, 
% %to improve the performance, 
% ii) consumes a lot of enclave memory to store HTs, and 
% iii) may require frequent EPC swapping, costing up to hundreds of thousands of cycles per swapping and incurring additional overhead \cite{dinh2019everything}. 

Here we propose a more efficient method. 
We thus introduce an alternative method to securely and efficiently make inference in the CSP host under the RF settings, namely SHE-based inference.
% main operations in HE-based inference
The primary operations include: 
\ding{182} DO encrypts the unlabelled instances with SHE and sends them to the host buffer;
\ding{183} enclave sends the encrypted HTs to the host \notewang{To-be-discussed} \notegio{This is exactly why it is not clear: from this sentence it looks like the enclave is "sending" something to a host and I do not thing that this is the right way of describing the passage between enclave computation and host computation environments} and is responsible \notegio{what is responsible? Do you mean to just updates some of the HTs?} for replacing the HTs if some of them are updated inside the enclave; 
\notewang{and provides the new encrypted HTs if some of them are updated (\ie HT keeps growing) in the following training.}
\ding{184} The host performs the homomorphic matrix multiplications and sends the results to DO;
\ding{185} DO decrypts the result matrices and the encrypted auxiliary information (\eg label array), then get the target label by comparing the elements in matrices with the labels in the array. 
\notegio{why is notable that they have the same representation?} \notewang{Because in the following, we will encrypt these matrices under SHE.} Notably, the instances and HTs are generated and represented in the same way as $\mathcal{M}_i$ and $\mathcal{M}_t$ in Section~\ref{sub:HT_inference}. 
%To protect the instances and HTs from CSP, we resort to SHE. 
% Considering that $M$ could be large, it incurs a performance penalty when performing homomorphic operations on multiple ciphertexts. 
% To address this issue, we introduce the ciphertext packing to reduce the expansion rate of ciphertexts and parallelize the homomorphic computations, thus achieving better performance in terms of amortized space and time complexity. 

% \paragraph{\textbf{HE-based Matrix Multiplication}}
% \noindent\textbf{HE-based Matrix Multiplication.}
\subsubsection{HE-based Matrix Multiplication}
\label{para:HEMatMul}
The na\"ive solution \notewang{to encrypt a matrix} \notegio{to do what?} is encrypting each row/column of the matrix (assume $s{\times}s$ square matrix) as a ciphertext (\ie $slots=s$, \notewang{the ciphertext contains $s$ values in $slots$}). \notegio{I do not know what this  $slots=s$ means.}
Subsequently, we perform HE multiplications between these ciphertexts, and finally sum the values in different slots by rotating them through the Frobenius Automorphisms \cite{wu2012using}. 
This solution requires $s^2$ multiplications, $s{\cdot}log(s)$ slot rotations and $2s$ ciphertexts, and it turns out to be too computational expensive.

% HE-based Multiplications
To improve the performance of performing matrix multiplications on packed homomorphic ciphertexts, we follow the method proposed in \cite{jiang2018secure}, \notewang{composed of matrix encoding, matrix encryption and matrix multiplication}.
\sout{We encode the matrices $\mathcal{M}_i$ and $\mathcal{M}_t$ into two ciphertexts, respectively, and then perform HE matrix multiplication between them as explained in the following.} \notegio{I do not understand what you mean with encoding the two matrices as two different ciphertexts...you need to explain a bit more.}

 
% \textit{Matrix encoding:} 
\noindent\textbf{Matrix encoding.}
We use a row ordering encoding map to transform a $s \times s$ square matrix $\mathcal{M}$ into a vector $vec$ of dimension $n=s^2$, \ie $vec$ is the concatenation of row vectors of $\mathcal{M}$. 
%In doing so, we get two ciphertexts with $slots=n$ respectively. 
Assume $(k{\leq}s){\wedge}(M{\leq}s)$ and $s$ is a power-of-two integer, in general, we can pad zeros at the end of each row to set $s$ as a power of two. 
Note that, in the following, multiple $\mathcal{M}_t$ can be packed into one matrix $\mathcal{M}$ if $slots$ is large enough. 
Here, we focus on encoding only one $\mathcal{M}_t$ for simplicity. 

% \textit{Matrix encryption:} 
\noindent\textbf{Matrix encryption.}
Given two encoded matrices (\ie $n$-dimensional vectors), we encrypt them into two ciphertexts with $slots=n$ respectively (see encryption details in Section~\ref{background:HE procedure}). 
Follow the options in \cite{jiang2018secure}, we provide two forms of ciphertext, namely \textit{pre-processed ciphertext} and \textit{normal ciphertext}. 
The former indicates that the ciphertext pre-computation is enabled and DO performs liner transformations on the encrypted $vec$ (\ie $\mathtt{LinearTrans({\sigma}(vec))}$) with some specified permutations, \ie ${\sigma}(vec)$. 
\notewang{For the normal ciphertext, we simply encrypt the $vec$ into a ciphertext without any extra operations.}
The reason of  generating pre-processed ciphertexts is to introduce more constant multiplications instead of homomorphic multiplications and reduce the number of slot rotations. 
It thus gives us a trade-off between space and time. 
In doing so, we can significantly speed up the homomorphic matrix multiplication but at the cost of memory usage increase (see the performance gap in Table~\ref{table:S3}). 
Here, we assume the ciphertext pre-computation is performed at DO side and the enclave only needs to output the \notegio{what is normal?} normal ciphertext(s). 

% \textit{Matrix multiplication:} 
\noindent\textbf{Matrix multiplication.}
The host computes the Hadamard multiplication between two ciphertexts $Ctxt.\mathcal{M}_i$ and $Ctxt.\mathcal{M}_t$, and finally aggregates all of the resulting ciphertexts. 
%Given two ciphertexts $Ctxt.\mathcal{M}_i$, we perform homomorphic matrix multiplications based on operations such as SIMD arithmetics, scalar multiplication, and ciphertext slot rotation. 
Theoretically speaking, the most expensive operations of performing such type of matrix multiplications are $s$ multiplications and $3s+5\sqrt{s}$ rotations. 
For more details about the procedure of matrix multiplication, we refer to \cite{jiang2018secure}.

% Theoretically speaking, the most expensive operations of performing such kind of matrix multiplications in our approach are ${\lceil}(K{\times}N_Q{\times}M^2)/{s^3}{\rceil}$ multiplications and $({\lceil}{K{\times}N_Q{\times}M^2{\times}(3s+2\sqrt{s})}/{s^4}{\rceil})$ rotations. 

% \paragraph{\textbf{HE Parameter Setting}}
\notewang{SHE }\noindent\textbf{Parameter Selection.}
\label{para:HE parameter}
\notegio{parameters for what?}
We first introduce several \sout{related} parameters \notewang{of SHE scheme to support homomorphic matrix multiplications} \notegio{related to what?}:
$m$, cyclotomic polynomial, defines $\phi(m)$; 
$p$, plaintext prime modulus; 
$bits$, number of bits of the modulus chain, indicates the ability of processing noise. 
The choice of these parameters determines the performance of our SHE-based solution and the security level.

To support homomorphic matrix multiplications, the matrix dimension should be a power-of-two integer (\eg $16{\times}16$, $32{\times}32$, $64{\times}64$ matrix). 
However, \sout{it is unavailable} \notewang{it is difficult} \notegio{what is unavailable?} to directly generate the ciphertext with exact slots (\eg $slots=256, 1024, 4096$) due to the interdependence between these parameters. 
For example, the number of multiplicative level reduces when increasing the parameters $m$ and $p$. 
Moreover, we have to select $m$ and $bits$ such that they guarantee at least 80-bit security level against the known attacks of the LWE problem \cite{albrecht2015concrete}. 
Additionally, the totient of $m$, $\phi(m)$, should be divisible by the number of slots (\eg $slots$ = 256). 
Finally, we select the plaintext prime modulus $p$ such that $\phi(m)/{\eta} = slots$, where $\eta$ is the multiplicative order of $p$ modulus $m$.

% \paragraph{\textbf{RF Inference}}
% \noindent\textbf{RF Inference.}
\subsubsection{RF Inference}
We give the detailed process described in Step \ding{182}-\ding{185}. 
DO selects the proper HE parameters based on the parameter setting to generate public key $he\_pk$ and secret key $he\_sk$, and then shares them with the enclave through the secure channel (described in Section~\ref{sub:setup}). 
DO packs the instances as $\mathcal{M}_i$, then encrypts it with $he\_pk$, finally sends it to the host buffer.
The enclave side first reconstructs the $he\_pk$ and $he\_sk$ based on shared HE contexts. 
The enclave generates the tree matrix $\mathcal{M}_t$ for each HT, then it encrypts all $\mathcal{M}_t$ with $he\_pk$, finally sends \notewang{To-be-discussed} \notegio{again the enclave is not sending anything to the host. it is more like passing in unsecure environment} them to the host.
\notegio{the text below needs to be better...}
\uline{As mentioned before, multiple $\mathcal{M}_t$ can be packed into one ciphertext as long as the $slots$ are enough. 
The number of the ciphertexts roughly depends on the $slots$ and the number of HTs. 
Once some of the HTs are updated, the enclave repeats the operations to output new encrypted matrices to replace the old ones. 
Finally, the host performs HE matrix multiplications and sends the results to DO. 
DO decrypts the result matrices to find the target labels based on the auxiliary information (\eg label arrays)}. 

%Note that we assume that $\mathcal{A}$ would not perform ciphertext manipulation, for example, dropping or duplicating ciphertext, to break data integrity in the \textit{CSP} in this HE-based setting.

==> sections/RF_details.tex <==





==> sections/RF_perf.tex <==
\subsection{Performance of RF Training and Inference}
\begin{figure*}[!ht]
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=1\linewidth]{graph/exp/RF_training_15_Tree50.eps}
                \caption{15-50}
                \label{fig9:RF1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=1\linewidth]{graph/exp/RF_training_15_Tree100.eps}
                \caption{15-100}
                \label{fig9:RF2}
        \end{subfigure}%
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=1\linewidth]{graph/exp/RF_training_31_Tree50.eps}
                \caption{31-50}
                \label{fig9:RF3}
        \end{subfigure}%
        \begin{subfigure}[b]{0.25\textwidth}
                \centering
                \includegraphics[width=1\linewidth]{graph/exp/RF_training_31_Tree100.eps}
                \caption{31-100}
                \label{fig9:RF4}
        \end{subfigure}
        \caption{The comparison of RF training with different feature-trees pairs (\ie number of features and trees)}\label{fig9}
\end{figure*}

\noindent\textbf{Performance of RF training.}
\notegio{the text in this section needs to be carefully checked and refined.}
\notewang{Example of ML papers setting: We use 50 and 100 random trees with the square root of the number of features as the fixed number of random features to split.}
To evaluate the performance of RF, the total number of features $d$ is set to 15 and 31 \notegio{One problem that i have with these numbers is that it is not explained why we have chosen them. I have said this earlier on} \notewang{To-be-discussed}, thus each tree has 4 and 6 features, respectively ($\sqrt{d}+1$) \notewang{(${\approx}\sqrt{d}$) \cite{breiman2001random}}. \notegio{I am not sure that this formula is correct here. please double check. Also why is it the case??? } 
We select the number of trees (\ie 50 and 100 \notewang{\cite{wu2020gpu,marron2014random}}) as the variant to observe the change of total runtime. 
\notewang{100 trees, if needed, I can provide those references which also adopt 100 trees (\ie GVFDT), but as discussed with Ocean, this number is very normal and no need to explain.}
\notegio{Remember that this is a security conference not a machine learning one. We need to say that this is the standard in the field at least or give some reference.}
In Fig.~\ref{fig9}, we observe a linear growth in training runtime with the increase of the number of samples (from $1{\times}10^4$ to $5{\times}10^4$). 
We are aware that by training RF on more trees and features, it would increase the total runtime, because there are more permutations between different features and consequently generate larger matrix \notegio{again is there only one single matrix?} \notewang{can be integrated into a single matrix during training}. 
Roughly speaking, given the number of trees $N_t$ and possible permutations between features $\pi(S_d)$ in each tree, we need to perform matrix multiplications between $N{\times}M$ data sample matrix and $M{\times}(N_t{\cdot}{\pi(S_d)})$ query matrix.

It shows that the obliviousness in our solution incurs negligible overheads.
Precisely, in Fig.~\ref{fig9:RF1} and~\ref{fig9:RF2}, \sys and $\mathtt{SGX~only}$ baseline have almost the same performance.
%Both of them incur around $6.5{\times}$ (50 trees) and $6.4{\times}$ (100 trees) additional overheads compared to \textit{Insecure} baseline. 
They are up to ${\thicksim}6.3{\times}$ faster than $\mathtt{Na{\ddot{\i}}vely~Oblivious~SGX}$.
In Fig.~\ref{fig9:RF3} and~\ref{fig9:RF4}, \sys is up to ${\thicksim}3{\times}$ (50 trees) and ${\thicksim}2.2{\times}$ (100 trees) faster than $\mathtt{Na{\ddot{\i}}vely~Oblivious~SGX}$ and slows down by ${\thicksim}2.1{\times}$ and ${\thicksim}1.5{\times}$ compared to $\mathtt{SGX~only}$ baseline.

%It increases by ${\thicksim}0.02{\times}$ to ${\thicksim}0.06{\times}$ and ${\thicksim}0.01{\times}$ to ${\thicksim}0.04{\times}$ for 15 features with 50 and 100 tree respectively. For 31 features, it increases by ${\thicksim}0.01{\times}$ to ${\thicksim}0.03{\times}$ and ${\thicksim}0.02{\times}$ to ${\thicksim}0.04{\times}$, compared to non-oblivious version. The small performance gap is because each tree has less features (such as 4 and 5), thus eliminates the influences of using oblivious primitives as much as possible.

\begin{figure}[!t]
\centering
\includegraphics[width=3.5in]{graph/exp/RF_evaluation.eps}
\caption{The Comparison of RF inference} 
\label{fig11}
\end{figure}

\noindent\textbf{Performance of RF inference.}
Regarding RF inference inside the enclave, as expected with the time consumption, our solution performs up to ${\thicksim}41{\times}$ and ${\thicksim}11{\times}$ better than $\mathtt{Na{\ddot{\i}}vely~Oblivious~SGX}$ (shown in Fig.~\ref{fig11}). 
Intuitively, by transforming each tree into a matrix, we get rid of the heavy usage of oblivious primitives (\eg $\mathtt{oaccess}$) during inference. 

\noindent\textbf{Performance of homomorphic matrix multiplication.}
Before introducing the performance of HE-based RF inference, we first quantify the performance gap between different matrix dimensions in homomorphic matrix multiplications.

\begin{table*}[!ht]
\centering
\footnotesize
 \caption{Performance of homomorphic matrix multiplication}
 \label{table:S3}
 \begin{ThreePartTable}
    \begin{tabular}{ccccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Dimension}} & \multicolumn{2}{c}{\textbf{Ciphertext Size (MB)}} & \multicolumn{2}{c}{\textbf{Encryption (s)}} & \multicolumn{2}{c}{\textbf{Decryption (s)}} & \multicolumn{2}{c}{\textbf{Matrix Multiplication (s)}} \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
        & \textbf{Pre-Ctxt} & \textbf{Ctxt} & \textbf{Pre-Ctxt} & \textbf{Ctxt} & \textbf{Pre-Ctxt} & \textbf{Ctxt} & \textbf{Pre-Ctxt} & \textbf{Ctxt} \\
        \midrule
        16 & 2.25  & 0.14 & 0.12 & 0.04 & 0.56 & 0.57 & 2.03 & 5.01 \\
        \hline
        32 & 16 & 0.5 & 0.24 & 0.06 & 1.56 & 1.57 & 1.67 & 4.48 \\
        \hline
        64 & 24 & 0.38 & 1.76 & 0.24 & 2.35 & 2.39 & 1.98 & 4.27 \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
    \centering
        \footnotesize
        \item \textbf{Pre-Ctxt}: Pre-processed ciphertext, significantly speeds up the matrix multiplication but with a larger ciphertext size. 
        \item \textbf{Ctxt}: Normal ciphertext, smaller size but consumes more matrix multiplication time.
    \end{tablenotes}
 \end{ThreePartTable}
\end{table*}

\begin{table*}[!ht]
\centering
\footnotesize
 \caption{Performance of SHE-based inference}
 \label{table:S4}
 \begin{ThreePartTable}
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Trees} & \textbf{Features} & \textbf{Host Runtime (min)} & \textbf{Enclave Runtime (s)} & \textbf{Communication Cost (MB)} \\
        \midrule
        % client runtime for 64 mat, 2.36s
        50 & 15  & 0.23 & 0.59 & 2.63 \\
        \hline
        100 & 15 & 0.43 & 1.09 & 4.88 \\
        \hline
        50 & 31  & 0.84 & 3.04 & 9.38 \\
        \hline
        100 & 31 & 1.68 & 6.00 & 18.76 \\
        \bottomrule
    \end{tabular}
 \end{ThreePartTable}
\end{table*}

The matrix dimension is set to 16, 32 and 64 in the following experiment, \ie $slots=256, 1024, 4096$. 
We present the timing results for encryption, decryption and matrix multiplication, as well as ciphertext size in Table~\ref{table:S3}. 
%Here, we provide two types of ciphertext, normal and pre-processed ciphertext. 
%For the pre-processed ciphertext, we pre-process the matrices in the cleartext and generate a set of ciphertexts, achieving a better performance (See Section~\ref{sub:RF_eva} for details). 
We use 16 threads to speed up the homomorphic computation since most operations can be highly parallelized. 
Notably, there is no much difference in performance between 8 and 16 threads when using $16{\times}16$ and $32{\times}32$ matrices. 
One can improve the performance using as many threads as possible when processing the ciphertexts with more slots.

Table~\ref{table:S3} shows that the use of ciphertext optimization improves the performance of matrix multiplication by roughly $2.47{\times}$, $2.68{\times}$ and $2.16{\times}$ when matrix dimension is 16, 32 and 64 respectively. 
However, it slows down the encryption by $3{\times}$, $4{\times}$ and $7.3{\times}$ and increases the ciphertext size by roughly $16{\times}$, $32{\times}$ and $63{\times}$. There is almost no difference between the decryption time. 
Overall, it gives us a trade-off between space and time. That is, we trade the communication cost at DO side with less HE matrix multiplication latency in our setting.

\noindent\textbf{Performance of HE-based RF inference}
In this section, we investigate the performance of running RF inference outside of the enclave. 
We adopt the $64{\times}64$ matrix in our following experiment as it only costs 1.98s and processes more data \ie 4096 slots. 
On the one hand, processing the HE ciphertext with optimization at the DO side allows us to trade off memory usage for run-time. 
On the other hand, we argue that DO can tolerate this memory usage since only a batch of instances is encrypted at a time. 
Next, we discuss the inference performance of using $64{\times}64$ matrix and leave the comparison of the other two matrices for future work. 

In Table~\ref{table:S4}, \textit{Host Runtime} is mainly composed of homomorphic matrix multiplication latency. 
\textit{Enclave Runtime} includes the matrix generation and encryption latency.
\textit{Communication Cost}, depending on the number of trees and features, as well as the chosen ciphertext, indicates the total size of HE ciphertexts.
The results show that it only costs around 0.43 min and 1.68 min to perform SHE-based inference for 100 trees. 
Since homomorphic matrix multiplication is the most costly operation compared to others (\eg encryption and decryption), we report it as the consumption of SHE-based inference.
Although it consumes more time than our oblivious solution and $\mathtt{Na{\ddot{\i}}vely~Oblivious~SGX}$, we argue that it is acceptable since we securely store the trees outside of the enclave and thus provide the inference service without consuming more enclave memory.
% so that give way for following training tasks

==> sections/background-backup-SHE-CP.tex <==
\subsection{Somewhat Homomorphic Encryption}
\label{background:HE procedure}

Homomorphic Encryption (HE) supports operations on encrypted data returning the encrypted results. 
HE makes it possible to outsource all of the computations to a third-party (e.g., a  cloud service) in a secure way. 
In this work, we employ Somewhat Homomorphic Encryption (SHE)  primitives \cite{brakerski2011fully,naehrig2011can} which supports a limited number of multiplications but it is more efficient than fully HE. 
%\notewang{HE is usually categorized as fully/somewhat/partial/level HE, somewhat HE is efficient than fully HE (FHE).}
%For the purpose of our work, the symmetric-key variant SHE suffices and we give the construction of symmetric-key $SHE=(KeyGen, Enc, Dec, Eval)$ based on \cite{brakerski2011fully}. 
SHE security is based on the Ring Learning With Errors (RLWE) assumption \cite{lyubashevsky2010ideal}.

\begin{itemize}
    \item $Setup$ Generate the cyclotomic polynomial $f(x)=x^n+1$ and the modulus $q$ where $n=2^{\kappa}$, $q{\equiv}1(mod\ 2n)$ and $\kappa$ is the security parameter. Subsequently, define a discrete Gaussian error distribution ${\chi}=D_{{{\mathbb{Z}}^n},{\sigma}}$ with a standard deviation $\sigma$. 
    %A additional parameter $D{\in}\mathbb{N}$ defines a bound on the maximum number of multiplications that can be performed correctly after homomorphic computations.
    
    Then define the rings as $R={\mathbb{Z}}_t[x]/f(x)$, the message space as $R_t={\mathbb{Z}}_t[x]/f(x)$ and the ciphertext space as $R_q=R/qR={\mathbb{Z}}_q[x]/f(x)$ where the prime $t<q$. Output public parameters $n, q, {\chi}$.
    
    \item $KeyGen(1^{\kappa})$ Generate the secret key $sk=s$ where sampling $s\stackrel{\$}{\leftarrow}{\chi}$. Set the public key $pk = (a_0, a_1)$ where $a_0 = -({a_1}s+te)$ and $e\stackrel{\$}{\leftarrow}{\chi}$.
    
    % \item $Enc_{sk}(m)$ Given $sk$ and $m{\in}R_t$, sample $a\stackrel{\$}{\leftarrow}R_q$ and $e\stackrel{\$}{\leftarrow}{\chi}$, output the ciphertext $ct=(c_0,c_1)=(as+te+m,-a){\in}R_q^2$.
    \item $Enc_{sk}(m)$ Given $sk$ and $m{\in}R_t$, sample ${u, f, g}\stackrel{\$}{\leftarrow}{\chi}$, output the ciphertext $ct=(c_0,c_1)=({a_0}u+tg+m,{a_1}u+tf){\in}R_q^2$.
    
    \item $Dec_{sk}(ct)$ Output the message $m=((c_0+c_1s)mod\ q) mod\ t$.
    
    \item $Eval(F;ct_1,{\cdots},ct_k)$ Given a set of ciphertexts $(ct_1,{\cdots},ct_k)$, output a ciphertext $ct^{\prime}$ based on the circuit $F:(R_t)^k{\rightarrow}(R_t)$. The details of homomorphic addition and multiplication in $R_t$ refer to \cite{brakerski2011fully,naehrig2011can}.
\end{itemize}

\subsection{Ciphertext Packing}

%\notegio{Does this technique apply to SHE as well? Do you have a specific reference?} 
%\notewang{Yes, it can be applied to SHE. (In fact, as long as it's based on RLWE assumption, the ciphertext packing can be applied to current HE systems.) We can add references as follows.}
Ciphertext packing technique plays a critical role in improving the performance of modern HE systems. 
Smart and Vercauteren \cite{smart2014fully} initiated the study of ciphertext packing based on polynomial-CRT (Chinese Remainder Theorem). 
Since then, it has been widely used in HE's variants (\eg SHE \cite{wu2012using,chen2020heaan,cheon2017homomorphic}) to implement the parallel computation based on ciphertexts.
It enables us to decompose the plaintext space $R_t$ into a vector of non-interacting \textit{plaintext slots}, denoted as $slots$. 
Specifically, given $slots$ messages $m_1{\in}R_{t1},{\cdots},m_{slots}{\in}R_{t(slots)}$, one can encode them into a single message $m{\in}R_t$ and encrypt it into a single ciphertext, and thus perform component-wise arithmetic operations over the slots in a SIMD (Single-Instruction Multiple-Data) manner \cite{wu2012using}.

%Hence, we can encrypt multiple plaintext values into a single ciphertext and leverage the Single-Instruction Multiple-Data (SIMD) technique \cite{smart2014fully} to perform homomorphic operations in batch. 

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discuss}
% Our experimental evaluation showed that:
% \begin{itemize}
%     \item Our prototype protects the privacy of data (including labelled and unlabelled data, and intermediate parameters), as well as the target model. 
%     The experimental results show that our solution outperforms na\"ive methods in either training or inference phase.
%     %We implemented it inside the enclave in a matrix-based method while introducing oblivious primitives to thwart access-pattern attack, thus keeping the HT structure private.
    
% \end{itemize}

In this section, we discuss the limitations of \sys, and provides some workarounds. 
\begin{itemize}
    \item The main limitation of the oblivious matrix-based method is that when the number of features increases the computation overhead becomes too prohibitive for practical purposes. To address this we outline two potential solutions. 
    %The experimental results show that our oblivious matrix-based method is limited to datasets with a lot of features. 
    %There are two interesting ways to further improve the performance: 
    1) Implementing multi-TEE by using GPU and CPU hardware features \cite{volos2018graviton}, where the GPU TEE executes the matrix multiplications to improve the performance \sout{and the SGX-based TEE mitigates the untrusted I/O operations} \notewang{and Telekine \cite{hunt2020telekine} is deployed to provide secure oblivious CPU-GPU communications}. 
    \notewang{Unfortunately, there are not currently any GPU TEEs on the market. We leave this for future work.}
    \notegio{I think we need to say that when the TEE on GPUs is avaiable...but again, is this an extension of our system or a complete new approach? I don't understand the part around SGX based TEE to mitigates the untrusted I/O. You cannot have untrusted I/O on GPUs?}
    %combining \textit{GPU-TEE} \cite{volos2018graviton} with \textit{CPU-TEE}.
    %Since the performance of our solution depends much on matrix multiplications that have inherently input-independent access patterns, GPU-TEE can significantly improve it while providing strong security guarantees. 
    %In addition, matrix multiplications have inherently input-independent access patterns in CPU-TEE and GPU-TEE.
    %and thus are especially suitable for GPU-enabled machines.
    \sout{2) leveraging hardware-based instructions (\eg SSE and AVX2) to accelerate the matrix multiplications inside the enclave.} \notegio{As a reviewer I would question why this has not been implemented in the current version.}
    \notewang{2) An alternative method is securely outsourcing linear operations (\ie matrix multiplications) to untrusted GPUs by employing lightweight cryptographic primitives (\ie secret sharing \cite{tramer2018slalom}).}
    % \item When dealing with a small number of features (\eg 7 features) using $64{\times}64$ matrix (\eg 4096 slots), it wastes too many slots (padded with zero). 
    % It may be possible to pack multiple matrices into $64{\times}64$ matrix among iterations.
    \item \sout{Increased noise in the ciphertexts may cause error decryption and extra computation overhead. Fortunately,} The hybrid privacy-preserving model (HE within SGX enclave) in our framework can integrate into HE computations to refresh the ciphertexts, which enable the system to eliminate the noise. 
    \notewang{We can manage HE calculations based on this model in CSP to avoid the operations of processing the noise from the HE ciphertexts, thus improve the performance of HE-based systems.}
    \sout{It can be further applied to HE-based systems that are deployed in cloud platforms to speed up HE computations.} 
    \notegio{If the noise is an issue why have you not addressed this already in the current implementation?}
    %for instance, refresh the ciphertexts (\ie eliminate the noise). 
    %This is because the increased noise in the ciphertexts probably leads to incorrect decryption and the solution, \textit{bootstrapping}, usually comes with heavy computation overhead. 
    %In such case, our hybrid model can be used to refresh the ciphertexts (\ie eliminate the noise) without leaking private data.
    %can be further used in ML domain with respect to the cloud computing.
    \item Introducing the Homomorphic Message Authentication Codes (HoMAC) \cite{catalano2013practical} as a building block to protect our SHE-based inference from the attacks that modify or replay the HE ciphertexts. \notegio{Is an attacker that modifies packets in transit part of our thread model? if not I think we need to be more precise. }
    \notewang{If the attacker is malicious, she can modify the ciphertexts. Currently, those available HE libraries didn't provide such integrity protection.}
    %in our SHE-based inference to ensure the computation integrity when performing HE operations in the CPU host. 
    \sout{In addition, since the ciphertexts are encrypted/decrypted by DO/enclave who are fully trusted in our work (see Section~\ref{threat model}), the homomorphic public key is unnecessary. We can further extend the HE constructions to symmetric-key variant to improve the performance.} \notegio{I do not understand how the public HE key is related to the fact that DO/Enclave are trusted. And if the symmetric-key variant exist why has not been used in the first place?}
    \notewang{Currently, those available (popular and famous, like IBM and Microsoft) HE libraries didn't provide such kind of variant. We need to integrate this part into current libraries. Maybe the security proof is also needed.}
    % we can further extend the HE constructions to symmetric-key variant since public key is unnecessary in our framework. 
    %\lei{please add the reason why you introduce the scheme here.} 
    %\lei{hard to understand why public key is unnecessary in our framework}
    
    \item \sout{Regarding RF implementation in \sys, we do not implement the module detecting concept drift and replacing HTs with the new ones. It can be further integrated into \sys in the future.} \notegio{I htink this is not a limitation of hte current system....have we even talked about concept drift as a feature of this system? If not, we should remove this part.}
    %Concept drift issue in ML is not considered in current framework, since our goal is focusing on features correct classification (\lei{I'm not sure, please correct it}). To mitigate the potential risk, we can integrate the scheme of subsequently replacing the HTs into the \sys to address the concept drift problem.  
\end{itemize}
